SPECTRE: Defending Against Backdoor Attacks Using Robust Statistics

Modern machine learning increasingly requires training on a large collection of data from multiple sources, not all of which can be trusted. A particularly concerning scenario is when a small fraction of poisoned data changes the behavior of the trained model when triggered by an attacker-specified watermark. Such a compromised model will be deployed unnoticed as the model is accurate otherwise. There have been promising attempts to use the intermediate representations of such a model to separate corrupted examples from clean ones. However, these defenses work only when a certain spectral signature of the poisoned examples is large enough for detection. There is a wide range of attacks that cannot be protected against by the existing defenses. We propose a novel defense algorithm using robust covariance estimation to amplify the spectral signature of corrupted data. This defense provides a clean model, completely removing the backdoor, even in regimes where previous methods have no hope of detecting the poisoned examples. Code and pre-trained models are available at https://github.com/SewoongLab/spectre-defense .

==> ideas.tex <==
Some future directions. 

1. Online defense against backdoor (has it been studied under FL backdoor?) 
- show it is effective
- restriction on defense: only access gradients over time
- can we still defend, in the end? (compare against sever).
Q. do we need the entire past gradients or can we just keep some hash?

2. Attribution and forensics: we need to give pre-defined scores, and efficient way to detect. Test loss on a subset as the score. 


3. Mathematical model that exhibits spectral signature. 

4. making detector small: 
- What happens with NTK, Gaussian kernels, 

5. Adversarial training: 


